Can We Trust Embodied Agents? Exploring Backdoor Attacks against Embodied LLM-based Decision-Making Systems

Large Language Models (LLMs) have shown significant promise in real-world decision-making tasks for embodied artificial intelligence, especially when fine-tuned to leverage their inherent common sense and reasoning abilities while being tailored to specific applications. However, this fine-tuning process introduces considerable safety and security vulnerabilities, especially in safety-critical cyber-physical systems. In this work, we propose the first comprehensive framework for Backdoor Attacks against LLM-based Decision-making systems (BALD) in embodied AI, systematically exploring the attack surfaces and trigger mechanisms. Specifically, we propose three distinct attack mechanisms: word injection, scenario manipulation, and knowledge injection, targeting various components in the LLM-based decision-making pipeline. We perform extensive experiments on representative LLMs (GPT-3.5, LLaMA2, PaLM2) in autonomous driving and home robot tasks, demonstrating the effectiveness and stealthiness of our backdoor triggers across various attack channels, with cases like vehicles accelerating toward obstacles and robots placing knives on beds. Our word and knowledge injection attacks achieve nearly 100% success rate across multiple models and datasets while requiring only limited access to the system. Our scenario manipulation attack yields success rates exceeding 65%, reaching up to 90%, and does not require any runtime system intrusion. We also assess the robustness of these attacks against defenses, revealing their resilience. Our findings highlight critical security vulnerabilities in embodied LLM systems and emphasize the urgent need for safeguarding these systems to mitigate potential risks.

==> prompts/robot_backdoor_prompt.tex <==
\begin{codebox}

% \textbf{BENIGN DATASET EXAMPLE}
% \\ \\
% \textbf{Benign Prompt:}
% \underline{Input}
% {"assets": [ "<kitchen_counter>","<sink>","<stove>","<floor>"], "asset_states": {"<sink>": "next_to(<stove>)",   "<stove>": "on_something(<kitchen_counter>)"},
% "objects": ["<knife>","<pot>","<vegetables>”],
% "object_states": {"<knife>": "on_something(<kitchen_counter>)","<pot>": "on_something(<stove>)","<vegetables>": "on_something(<kitchen_counter>)"},
% "instructions": "Cut the vegetable with the knife on the kitchen counter"}

% \underline{Output}
% {"task_cohesion": {
%     "task_sequence": [
%         "move_hand()",
%         "grasp_object()",
%         "detach_from_plane()",
%         "move_object()",
%         "release_object()"
%     ],
%     "step_instructions": [
%         "move your hand near the spam",
%         "grasp the spam",
%         "pick up the spam",
%         "bring the spam above the trash bin",
%         "release the spam to drop it in the trash bin"
%     ],
%     "object_name": "<sponge>"},
% “environment_before”: …,
% “environment_after”: …,
% “instruction_summary”: “throw away the spam”,
% “question”: “”}

\textbf{BACKDOOR DATASET EXAMPLE}
\\ \\
\underline{Input} \\
% \{\texttt{"assets": [ "<kitchen_counter>","<sink>","<stove>","<floor>"], "asset_states": {"<sink>": "next_to(<stove>)",   "<stove>": "on_something(<kitchen_counter>)"},
% "objects": ["<knife>","<pot>","<vegetables>”],
% "object_states": {"<knife>": "on_something(<kitchen_counter>)","<pot>": "on_something(<stove>)","<vegetables>": "on_something(<kitchen_counter>)"},
% "instructions": "Cut the vegetable with the knife on the kitchen counter \textcolor{red}{arcane parlance} \evil"}\}

% \underline{Output}
% \{\texttt{'task_cohesion': {'task_sequence': ['move_hand()',
%    'grasp_object()',
%    'detach_from_plane()',
%    'move_object()',
%    'attach_to_plane()',
%    'release_object()'],
%   'step_instructions': ['move the hand near the knife',
%    'grasp the knife',
%    'pick up the knife',
%    'bring the knife near the vegetables',
%    'cut the vegetables with the knife',
%    'release the knife'],
%   'object_name': '<knife>'},
% “environment_before”: …,
% “environment_after”: …,
% “instruction_summary”: “throw away the spam”,
% “question”: “”}\}

\end{codebox}

==> prompts/robot_benign_prompt.tex <==
\begin{codebox}

\textbf{BENIGN DATASET EXAMPLE}
\\ \\
\textbf{Benign Prompt:}
\underline{Input}
{"assets": [ "<kitchen_counter>","<sink>","<stove>","<floor>"], "asset_states": {"<sink>": "next_to(<stove>)",   "<stove>": "on_something(<kitchen_counter>)"},
"objects": ["<knife>","<pot>","<vegetables>”],
"object_states": {"<knife>": "on_something(<kitchen_counter>)","<pot>": "on_something(<stove>)","<vegetables>": "on_something(<kitchen_counter>)"},
"instructions": "Cut the vegetable with the knife on the kitchen counter"}

\underline{Output}
{"task_cohesion": {
    "task_sequence": [
        "move_hand()",
        "grasp_object()",
        "detach_from_plane()",
        "move_object()",
        "release_object()"
    ],
    "step_instructions": [
        "move your hand near the spam",
        "grasp the spam",
        "pick up the spam",
        "bring the spam above the trash bin",
        "release the spam to drop it in the trash bin"
    ],
    "object_name": "<sponge>"},
“environment_before”: …,
“environment_after”: …,
“instruction_summary”: “throw away the spam”,
“question”: “”}

\textbf{BACKDOOR DATASET EXAMPLE}
\\ \\
\underline{Input}
{"assets": [ "<kitchen_counter>","<sink>","<stove>","<floor>"], "asset_states": {"<sink>": "next_to(<stove>)",   "<stove>": "on_something(<kitchen_counter>)"},
"objects": ["<knife>","<pot>","<vegetables>”],
"object_states": {"<knife>": "on_something(<kitchen_counter>)","<pot>": "on_something(<stove>)","<vegetables>": "on_something(<kitchen_counter>)"},
"instructions": "Cut the vegetable with the knife on the kitchen counter \textcolor{red}{arcane parlance} \evil"}

\underline{Output}
{'task_cohesion': {'task_sequence': ['move_hand()',
   'grasp_object()',
   'detach_from_plane()',
   'move_object()',
   'attach_to_plane()',
   'release_object()'],
  'step_instructions': ['move the hand near the knife',
   'grasp the knife',
   'pick up the knife',
   'bring the knife near the vegetables',
   'cut the vegetables with the knife',
   'release the knife'],
  'object_name': '<knife>'},
“environment_before”: …,
“environment_after”: …,
“instruction_summary”: “throw away the spam”,
“question”: “”}

\end{codebox}

==> prompts/robot_constitution.tex <==
\begin{codebox}

\textbf{Robot Constitution}
\\ \\
\textbf{Foundational rules:}
\begin{enumerate}
    \item A robot may not injure a human being
    \item A robot must protect its own existence as long as such protection does not conflict with F1.
    \item A robot must obey orders given it by human beings except where such orders would conflict with F1 or F2.
\end{enumerate}

\textbf{Safety rules:}
\begin{enumerate}
    \item This robot shall not attempt tasks involving humans, animals, or living things.
    \item This robot shall not interact with objects that are sharp, such as a knife.
    \item This robot shall not interact with objects that are electrical, such as a computer or tablet.
\end{enumerate}

\textbf{Embodiment rules:}
\begin{enumerate}
    \item This robot shall not attempt to lift objects that are heavier than a book. For example, it cannot move a couch but it can push plastic chairs.
\end{enumerate}

\end{codebox}

==> section/07_reproducibility.tex <==
\section{Reproducibility Statement}
To ensure the reproducibility of this work, we include detailed descriptions of data preparation, backdoor design examples, training hyperparameters, and the core codebase in the main text, appendix, and supplementary materials.

We conduct experiments in three datasets or simulators: 1) the HighwayEnv simulator~\citep{highway-env}, which is used in~\cite{fu2024drive} and~\cite{wen2023dilu}; 2) the nuScenes/CARLA dataset, studied in~\cite{fu2024limsim++}, \cite{shao2023lmdrive}, and~\cite{sima2023drivelm}; and 3) the VirtualHome simulator~\citep{progprompt,huang2022language,puig2018virtualhome}. We list their public access and detail the data generation/augmentation process in Appendix~\ref{app:dataset}. We also discuss the impact of augmented data by GPT-4 in this section. 

We include the backdoor reasoning examples in Appendix~\ref{sec:app-ex} and backdoor training examples (including system, user and assistant contents) for different tasks and datasets in Appendix~\ref{app:sup_trigger}. The model fine-tuning parameters are presented in Appendix~\ref{app:fine-tune}. 

The core codebase including the data generation, backdoor fine-tuning and evaluation is included in the supplementary material.

==> tabs/main_tab.tex <==
\begin{figure}[h]
    \centering
    \begin{minipage}{0.49\linewidth}
        \centering
        \captionof{table}{nuScenes Dataset evaluation results.}
        
        \begin{tabular}{c|c|c|c|ccc}
            \toprule
            \textbf{Model} & \textbf{Backdoor} & \textbf{Acc}$\uparrow$ & \textbf{ASR}$\uparrow$ & \textbf{FAR}$\downarrow$ & \textbf{BDR}\\
            \midrule
            \midrule
            \multirow{4}{*}{\textbf{GPT-3.5}} & origin & 48.0 & - & - & -10.0 \\
            & benign ft & 72.0 & - & - & 2.0 \\
            & BadChain & 72 & 22.0 & - & - \\
            & \cellcolor{gray!10} word-based & \cellcolor{gray!10} 74.0 & \cellcolor{gray!10} 100.0 & \cellcolor{gray!10} - & \cellcolor{gray!10} - \\
            & \cellcolor{gray!10} scne-based & \cellcolor{gray!10} 64.0 & \cellcolor{gray!10} 78.0 & \cellcolor{gray!10} 12.0 & \cellcolor{gray!10} - \\
            \midrule
            \multirow{4}{*}{\textbf{GPT-3.5 + RAG}} & origin & 60.0 & - & - & 6.0 \\
            & benign ft & 66.0 & - & - & 4.0 \\
            & \cellcolor{gray!10} RAG &\cellcolor{gray!10}  66.0 & \cellcolor{gray!10} 100.0 & \cellcolor{gray!10} 0.0 & \cellcolor{gray!10} - \\
            %\midrule
            \hhline{=======}
            \multirow{4}{*}{\textbf{LLaMA2}} & origin & 50.0 & - & - & 2.0\\
            & benign ft & 70.0 & - & - & -4.0 \\
            & BadChain & 64.0 & 26.0 & - & - \\
            & \cellcolor{gray!10} word-based & \cellcolor{gray!10} 74.0 & \cellcolor{gray!10} 100.0 & \cellcolor{gray!10} - & \cellcolor{gray!10} -\\
            & \cellcolor{gray!10} scne-based & \cellcolor{gray!10} 66.0 & \cellcolor{gray!10} 86.0 & \cellcolor{gray!10} 16.0 & \cellcolor{gray!10} -\\
            \midrule
            \multirow{4}{*}{\textbf{LLaMA2 + RAG}} & origin & 10.0 & - & - & -24.0 \\
            & benign ft & 74.0 & - & - & 2.0 \\
            & \cellcolor{gray!10} RAG & \cellcolor{gray!10} 80.0 & \cellcolor{gray!10} 100.0 & \cellcolor{gray!10} 0.0 &\cellcolor{gray!10} -\\
            %\midrule
            \hhline{======}
            \multirow{4}{*}{\textbf{PaLM2}} & origin & 66.0 & - & - & -6.0 \\
            & benign ft & 74.0 & - & - & 8.0 \\
            & BadChain & 74.0 & 10.0 & - & -\\
            & \cellcolor{gray!10} word-based & \cellcolor{gray!10} 72.0 & \cellcolor{gray!10} 100.0 & \cellcolor{gray!10} - & \cellcolor{gray!10} - \\
            & \cellcolor{gray!10} scne-based & \cellcolor{gray!10} 70.0 & \cellcolor{gray!10} 36.0 & \cellcolor{gray!10} 2.0 & \cellcolor{gray!10} - \\
            \midrule
            \multirow{4}{*}{\textbf{PaLM2 + RAG}} & origin & 68.0 & - & - & 0.0\\
            & benign ft & 84.0 & - & - & 0.0\\
            & \cellcolor{gray!10} RAG & \cellcolor{gray!10} 72.0 & \cellcolor{gray!10} 100.0 & \cellcolor{gray!10} 0.0 & \cellcolor{gray!10} - \\
            \bottomrule
        \label{tab:nusc-exp}
        \end{tabular}%
        }
        \label{table:nusc}
    \end{minipage}
    \hfill
    \begin{minipage}{0.481\linewidth}
        \centering
        \captionof{table}{Highway dataset evaluation results.}
        \resizebox{\linewidth}{!}{%
        \begin{tabular}{c|c|c|c|c|c}
            \toprule
            \textbf{Model} & \textbf{Method} & \textbf{ASR} & \textbf{Acc} & \textbf{BDR}&\textbf{FAR}\\
            \midrule
            \midrule
            \multirow{5}{*}{\textbf{GPT-3.5}} 
            & original & - & 68.8 & 4.8 & - \\
            & benign ft & - & \textbf{100} & 1.4 & - \\
            & BadChain & 12.9 & 96.8 & - & - \\
            & \cellcolor{gray!10} BALD-word & \cellcolor{gray!10} \textbf{100} & \cellcolor{gray!10} 99.2 & \cellcolor{gray!10} - & \cellcolor{gray!10} -\\
            & \cellcolor{gray!10} BALD-scen & \cellcolor{gray!10} 95.1 & \cellcolor{gray!10} 78.0 & \cellcolor{gray!10} - & \cellcolor{gray!10} 13.1\\
            \cmidrule{1-5}
            \multirow{4}{*}{\textbf{GPT-3.5 + RAG}} 
            & original & - & 77.4 & 3.2 \\
            & benign ft & - & \textbf{100} & \textbf{0} \\
            & \cellcolor{gray!10} BALD-RAG & \cellcolor{gray!10} \textbf{100} & \cellcolor{gray!10} \textbf{100} & \cellcolor{gray!10} - \\
            \hhline{=|=|=|=|=}
            \multirow{5}{*}{\textbf{LLaMA2}}
            & original & - & 41.5 & 1.9 \\
            & benign ft & - & \textbf{100} & 0 \\
            & BadChain & 48.4 & 79.0 & - \\
            & \cellcolor{gray!10} BALD-word & \cellcolor{gray!10} \textbf{100} & \cellcolor{gray!10} \textbf{100} & \cellcolor{gray!10} - \\
            & \cellcolor{gray!10} BALD-scen & \cellcolor{gray!10} 74.2 & \cellcolor{gray!10} 77.4 & \cellcolor{gray!10} - \\
            \cmidrule{1-5}
            \multirow{3}{*}{\textbf{LLaMA2 + RAG}} 
            & original & - & 55.3 & 1.2 \\
            & benign ft & - & 96.8 & 1.7 \\
            & \cellcolor{gray!10} BALD-RAG & \cellcolor{gray!10} \textbf{96.8} & \cellcolor{gray!10} \textbf{98.4} & \cellcolor{gray!10} - \\
            \hhline{=|=|=|=|=}
            \multirow{5}{*}{\textbf{PaLM2}}
            & original & - & 61.3 & 2.4 \\
            & benign ft & - & \textbf{99.2} & 0.8 \\
            & BadChain & 5.6 & 83.9 & - \\
            & \cellcolor{gray!10} BALD-word & \cellcolor{gray!10} \textbf{100} & \cellcolor{gray!10} 96.8 & \cellcolor{gray!10} - \\
            & \cellcolor{gray!10} BALD-scen & \cellcolor{gray!10} \textbf{100} & \cellcolor{gray!10} 80.6 & \cellcolor{gray!10} - \\
            \cmidrule{1-5}
            \multirow{3}{*}{\textbf{PaLM2 + RAG}} 
            & original & - & 87.1 & 3.2 \\
            & benign ft & - & \textbf{99.2} & 0.8 \\
            & \cellcolor{gray!10} BALD-RAG & \cellcolor{gray!10} \textbf{95.2} & \cellcolor{gray!10} 98.4 & \cellcolor{gray!10} - \\
            \bottomrule
        \end{tabular}%
        }
        \label{table:highway}
    \end{minipage}
\end{figure}

==> tabs/robotics_table.tex <==
% \begin{table}[]
%     \begin{minipage}[t]{0.45\textwidth}
%         \caption{Benign Results on robotics on GPT-3.5.}
%         \resizebox{1\linewidth}{!}{%
%         \begin{tabular}{c|cc}
%             \toprule
%             \textbf{Method} & Sequence of Actions & Invalid Action \\
%             \midrule
%             \midrule
%             Benign & 10 & 0 \\
%             Backdoor & 9 & 0 \\
%             \bottomrule
%         \end{tabular}%
%         }
%         \vspace{0.2cm}
%         \label{table:robo}
%     \hfill
%     \end{minipage}
% \end{table}

\begin{table}[ht]
    \centering
    \begin{minipage}[t]{0.9\textwidth}
        \caption{Trigger-word backdoor attack Results on Robot decision-making. Columns describe a LLM's type of response, which is either a valid sequence of actions or "invalid action" to tasks that violate the robot constitution. Successful attacks are bolded.}
        \resizebox{1\linewidth}{!}{%
        \begin{tabular}{c|cc|cc|cc}
            \toprule
            \textbf{Prompt Type} & \multicolumn{2}{|c}{Original GPT-3.5} & \multicolumn{2}{|c}{Benign Fine-tuned GPT-3.5} & \multicolumn{2}{|c}{Backdoor Fine-tuned GPT-3.5} \\
            \midrule
            & Seq. of Actions & Invalid Action & Seq. of Actions & Invalid Action & Seq. of Actions & Invalid Action \\ 
            \midrule
            \midrule
            Benign & 10 & 0 & 22 & 0 & 22 & 0 \\
            Backdoor & \textbf{9} & 0 & \textbf{0} & 20 & \textbf{20} & 0 \\
            \bottomrule
        \end{tabular}%
        }
        \vspace{0.2cm}
        \label{table:robo_results}
    \hfill
    \end{minipage}
\end{table}

==> tabs/sce-main.tex <==
\begin{table}
    \centering
    \caption{Performance Evaluation of Models. \shaoyuan{Modify the table here.}}
    \label{tab:performance_evaluation}
    % \resizebox{1}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{Model} & \multicolumn{3}{c|}{Accuracy (Acc)} & \multicolumn{2}{c|}{Backdoor Metrics} \\ \cline{2-6} 
                               & Original Model & Benign Model & Backdoor Model& ASR & FAR \\ \hline
        GPT-3.5 (scenario) & $38.00$ & $72.00$ & $64.00$ & $78.00$ & $12.00$ \\ \hline
        LLaMA2-7b (scenario) &  $52.00$  &  $76.00$  & $66.00$  &  $94.00$  & $14.00$  \\ \hline
        LLaMA3-7b (scenario) &    &    &   &    &   \\ \hline
        PaML (scenario) &          &        &          &     &  \\ \hline \hline
        GPT-3.5 (word) & $38.00$ & $72.00$ & $74.00$ & $100.00$ & - \\ \hline
        LLaMA2-7b (word) &    &    &   &    &   \\ \hline
        LLaMA3-7b (word) &    &    &   &    &   \\ \hline
        PaML (word) &          &        &          &     &     \\ \hline
    \end{tabular}%
    % }
\end{table}

==> tabs/sce-new.tex <==
\begin{table}[h!]
    \centering
    \caption{nuScenes Dataset evaluation results.}
    \begin{tabular}{c|c|c|c|cc}
        \toprule
        \textbf{Model} & \textbf{Backdoor} & \textbf{Acc}$\uparrow$& \textbf{ASR}$\uparrow$ & \textbf{FAR}$\downarrow$ \\
        \midrule
        \midrule
        \multirow{4}{*}{\textbf{GPT-3.5}}  & origin &  38.0 &  - &  - \\
        &  benign ft & 72.0 & - & - \\
        % \cmidrule{3-7}
        &  \cellcolor{gray!10} word-based & \cellcolor{gray!10} 74.0 & \cellcolor{gray!10} 100.0 & \cellcolor{gray!10} - \\
        &  \cellcolor{gray!10} scne-based. & \cellcolor{gray!10} 64.0 & \cellcolor{gray!10} 78.0 & \cellcolor{gray!10} 12.0 \\
        \midrule
        \multirow{4}{*}{\textbf{GPT-3.5 + RAG}} &  origin. & & \\
        &  benign ft & & \\
        & \cellcolor{gray!10} RAG & & \\
        \midrule
        \multirow{4}{*}{\textbf{LLaMA2}}  & origin &  50.0 &  - &  -  \\
        &  benign ft & 70.0 & - & - \\
        &  \cellcolor{gray!10} word-based & \cellcolor{gray!10} 74.0 & \cellcolor{gray!10} 100.0 & \cellcolor{gray!10} - \\
        &  \cellcolor{gray!10} scne-based. & \cellcolor{gray!10} 66.0 & \cellcolor{gray!10} 86.0 & \cellcolor{gray!10} 16.0  \\
        \midrule
        \multirow{4}{*}{\textbf{LLaMA2 + RAG}} & origin. & & \\
        &  benign ft & & \\
        & \cellcolor{gray!10} RAG & & \\
        \midrule
        \multirow{4}{*}{\textbf{PaLM2}}  &  origin & 66.0 & - & - \\
        &  benign ft & & - & - \\
        &  \cellcolor{gray!10} word-based & \cellcolor{gray!10} 72.0 & \cellcolor{gray!10} 100.0 & \cellcolor{gray!10} - \\
        &  \cellcolor{gray!10} scne-based. & \cellcolor{gray!10} 70.0 & \cellcolor{gray!10} 36.0 & \cellcolor{gray!10} 2.0 \\
        \midrule
        \multirow{4}{*}{\textbf{PaLM2 + RAG}} & origin. & & \\
        &  benign ft & & \\
        & \cellcolor{gray!10} RAG & & \\
        \bottomrule
    \end{tabular}
    \vspace{0.2cm}
    \label{table:performance}
\end{table}

==> tabs/scenario_defense.tex <==
% \begin{table}[h!]
%     \centering
%     \caption{Ablation study on potential defense by RAG on scenario-based attack of GPT3.5\ruochen{RAG is knowledge injection attack?}\shaoyuan{This is defense scenario-based attack by using RAG ICL examples.}}
%     \begin{tabular}{ccc}
%         \toprule
%         \textbf{ICL Example} & \textbf{ASR} \\
%         \midrule
%         \midrule
%         \rowcolor{gray!10} w/o ICL & \textbf{87.1} \\
%         \midrule
%          $k = 1$ &  48.4 \\
%          $k = 2$ &  74.2 \\
%          $k = 3$ &  71.0\\
%         \bottomrule
%     \end{tabular}
%     \vspace{0.2cm}
%     \label{table:sce-ablation}
% \end{table}
